The Conceptual VAE

In this report we present a new model of concepts, based on the framework of variational autoencoders, which is designed to have attractive properties such as factored conceptual domains, and at the same time be learnable from data. The model is inspired by, and closely related to, the Beta-VAE model of concepts, but is designed to be more closely connected with language, so that the names of concepts form part of the graphical model. We provide evidence that our model -- which we call the Conceptual VAE -- is able to learn interpretable conceptual representations from simple images of coloured shapes together with the corresponding concept labels. We also show how the model can be used as a concept classifier, and how it can be adapted to learn from fewer labels per instance. Finally, we formally relate our model to Gardenfors' theory of conceptual spaces, showing how the Gaussians we use to represent concepts can be formalised in terms of "fuzzy concepts" in such a space.

==> compositional-section.tex <==

\subsection{Composing Concepts}

In \citeA{tull2021categorical} our definition of fuzzy concepts is also extended to more general fuzzy \emph{conceptual processes} which transform concepts on one conceptual space to another, and formally define a \emph{symmetric monoidal category}. This builds on the earlier categorical treatment of crisp concepts in \citeA{bolt2019interacting}. 

The categorical approach allows us to reason about and \emph{compose} concepts using simple \emph{string diagrams}. For example, the concepts in this work are given by composing  concepts from each domain, so that \eqref{eq:factored-concept-density} becomes the following diagram. 
\[
\input{C-factored.tikz}
\]
However, more general concepts on the overall space need not factor as above. For example, we might imagine a \emph{rainbow} concept, which correlates position and colour according to the colours of the rainbow:
\begin{equation} \label{eq:rainbow}
%\includegraphics[scale=0.12]{figs/rainbow.png}
\input{rainbow1.tikz}
\end{equation} 
Thus the concept is satisfied by red shapes at the top, green shapes in the centre and blue shapes at the bottom (see Figure \ref{fig:rainbow-concept}). 

\begin{figure} 
\centering
    \includegraphics[]{figs/180_red_large_square_top.png}
    \includegraphics[]{figs/173_orange_large_triangle_top.png}
    \includegraphics[]{figs/156_green_medium_triangle_centre.png}
    \includegraphics[]{figs/242_indigo_small_circle_bottom.png}
    \includegraphics[]{figs/273_violet_small_circle_bottom.png}
    \caption{Example images for the `rainbow' concept.} 
    \label{fig:rainbow-concept}
\end{figure}

The diagrammatic approach is useful for combining these more general concepts, which we hope to explore in future (see Section \ref{sec:further_work}). A common approach is to use their pointwise product, which appears in diagrams through white `copying' dots. In \citeA{bolt2019interacting} these combinations are applied to crisp concepts to give conceptual semantics for natural language, by converting sentences into concepts diagrammatically as below.  Note that these diagrammatic concept combinations do not require any learning beyond the concepts themselves (assuming the string diagrams are given).
\begin{equation} \label{eq:DisCoDiag}
\includegraphics[scale=0.18]{figs/3.png}
= 
\includegraphics[scale=0.18]{figs/4.png}
\end{equation} 



% For example, a common approach is to use their pointwise product, which appears in diagrams through white `copying' dots.
% \eqref{eq:DisCoDiag}.
% The diagrammatic approach is useful for combining these more general concepts, which we hope to explore in future (see Section \ref{sec:further_work}). 
%It would be interesting to explore the learning of non-factored concepts such as \eqref{eq:rainbow} in our setup, as well as the effectiveness of the categorical composition procedures for concepts in \eqref{eq:DisCoDiag}. Beyond this, 
% which form a \emph{symmetric monoidal category}. It would be interesting to explore the learning of such conceptual processes, including for example ``metaphorical" mappings between domains. 
%  Furthermore, the categorical approach allows us to reason about and \emph{compose} concepts using simple \emph{string diagrams}. 
 % suggested in \citeA{tull2021categorical}. 
% This allows one to reason about and \emph{compose} concepts using  \emph{string diagrams}, building on the earlier approach of \citeA{bolt2019interacting}. 
% such as \eqref{eq:rainbow} in our setup, as well as the effectiveness of the categorical composition procedures for concepts in \eqref{eq:DisCoDiag}. Beyond this, the categorical approach allows one to explore the learning of conceptual processes between domains, such as the ``metaphorical" mappings suggested in \citeA{tull2021categorical}. 
% here all factor 
% which transform concepts on one conceptual space to another, and formally define a \emph{symmetric monoidal category}. This builds on the earlier categorical treatment of crisp concepts in \citeA{bolt2019interacting}. 
% The categorical approach allows us to reason about and \emph{compose} concepts using simple \emph{string diagrams}. 
% For example, the concepts in this work are given by composing  concepts from each domain, so that \eqref{eq:factored-concept-density} becomes the following diagram. 
% However, more general concepts on the overall space need not factor as above. For example, we might imagine a \emph{rainbow} concept, which correlates position and colour according to the colours of the rainbow:
% Thus the concept is 
\[
\input{C-factored.tikz}
\]
\begin{equation} \label{eq:rainbow}
\input{rainbow1.tikz}
\end{equation} 



==> name.tex <==
\section{A Formal Model of Concepts}
\label{sec:formal}

\Stevemar{ we should start with a line or two about why a formal treatment of the model is a good thing to do and cite Sean's existing papers straight away if this essentially repeats what's there; at least make the connection clear }




Here we outline the theoretical background for our work, based on a formalisation of \Gardenfors' framework of \emph{conceptual spaces} \cite{gardenfors,gardenfors2014}, which models conceptual reasoning in human and artificial cognition. A central claim of \Gardenfors' framework is that concepts should be represented as \emph{convex} regions of a space. While numerous formalisations of the theory have been presented, our work is based on the recent \emph{categorical} approaches from \cite{bolt2019interacting,tull2021categorical} which emphasize the \emph{compositional} aspects of the theory, and which we summarise here.


\begin{definition} 
A \emph{conceptual space} is a set $Z$ in which we may take convex combinations of elements. That is, for all $z_1,\dots,z_n \in Z$ and $p_1, \dots, p_n \in [0,1]$ with $\sum^n_{i=1} p_i = 1$ there is an element of $Z$ denoted
\[
\sum^n_{i=1} p_i \cdot z_i 
\]
%Todo: add citation. 
These convex combinations satisfy the rules one might expect; see \cite{bolt2019interacting} for a more precise formulation.
Additionally we require that $Z$ forms a \emph{measure space}, meaning it comes with a $\sigma$-algebra $\Sigma_Z$ of measurable subsets $M \subseteq Z$, and a measure $\mu \colon \Sigma_Z \to [0,\infty]$.  
\end{definition} 







% \begin{definition} 
% A \emph{convex set} is a set $Z$ in which we may take finite convex combinations of elements. That is, for all $z_1,\dots,z_n \in Z$ and $p_1, \dots, p_n \in [0,1]$ with $\sum^n_{i=1} p_i = 1$ there is an element of $Z$ denoted
% \[
% \sum^n_{i=1} p_i \cdot z_i 
% \]
% %Todo: add citation. 
% These convex combinations satisfy the rules one might expect; see \cite{bolt2019interacting} for a more precise formulation. A subset $A \subseteq Z$ is called \emph{convex} when it is closed under convex combinations of elements. 
% \end{definition} 

% For the purposes of this work, a conceptual space may be defined as follows. 

% %Todo: In fuzzy concepts paper, these were just measurable spaces (no fixed measure). But since we like densities here. 
% \begin{definition} 
% A \emph{conceptual space} is a convex set $Z$ which is also a \emph{measure space}. That is, it comes with a $\sigma$-algebra $\Sigma_Z$ of \emph{measurable} subsets, with a \emph{measure} $\mu \colon \Sigma_Z \to [0,\infty]$.  
% \end{definition} 

% Typically in \Gardenfors' theory, each conceptual space is composed from simpler factors called \emph{domains}. 

Typically a conceptual space is given as a product of simpler factors called \emph{domains}. That is, we have 
\[
Z = D_1 \otimes \dots \otimes D_n
\]
for domains $D_1,\dots,D_n$, which are themselves conceptual spaces.  Here we define $X \otimes Y = X \times Y$ with element-wise convex operations. 



Though they can be abstract, all the conceptual spaces and domains we consider here are of the following concrete form. 

%Todo: Double check that Lebesgue measures are closed under products. Or are they not? If not may need to use Borel version. 
\begin{example} \label{ex:RnCS}
Any convex subset $Z \subseteq \mathbb{R}^n$ forms a conceptual space. Here we equip $Z$ with the standard Lebesgue measure $\mu(A) = \int_A dz$ on $\mathbb{R}^n$. 
\end{example} 

% \[
% \sum_i p_i (x_i,y_i) := (\sum_i p_i x_i, \sum_i p_i y_i)
% \] 
% In this work all domains and conceptual spaces are subsets of $\mathbb{R}^n$ as in Example \ref{ex:RnCS}. 


Having defined conceptual spaces let us now consider concepts themselves. 

\begin{definition} 
A \emph{crisp concept} in a conceptual space $Z$ is a measurable  subset $C \subseteq Z$ which is \emph{convex}, meaning it is closed under convex combinations. 
\end{definition} 

We think of a point $z \in Z$ as belonging to the region $C$ of a crisp concept whenever  it forms an \emph{instance} or \emph{exemplar} of the concept. Convexity means that any point lying `in-between' two instances will again belong to the concept. \Gardenfors{} justifies convexity based on cognitive experiments, including evidence from the division of colour space in various cultures, and the relative ease of learning convex regions.


\begin{example} From \cite{bolt2019interacting}. For a simple example of a `colour' domain we can use the RGB \emph{colour cube}
\[
[0,1]^3 = \{(R,G,B) \mid 0 \leq R,G,B \leq 1\} \subseteq \mathbb{R}^3
\]
 depicted below, along with 
examples for crisp concepts `yellow' and `green'.
\[
\includegraphics[scale=0.2]{figs/1.png}
\]
% \[
% \includegraphics[scale=0.2]{figs/2.png}
% \]
\end{example} 


% The fact that such conceptual regions should be convex is argued by \Gardenfors' based on cognitive experiments, including evidence from the division of colour space in various cultures, as well as based on the easy learnability of convex regions. Indeed, convex regions of $ \mathbb{R}^n$ may be formed readily by taking the \emph{convex hull} $C= \mathsf{Conv}(\{z_1,\dots,z_n\})$ of a set of exemplars $z_1, \dots, z_m \in C$. 

% Given a set of exemplars of distinct concepts, the \emph{Voroni tesselation} provides a recipe for dividing up a Euclidean space into non-overlapping convex regions, each containing precisely one such exemplar. Such a process may be used by humans, for example when dividing colour space into distinct colour concepts using a set of exemplars of each colour. 

\subsection{Fuzzy Concepts}

The concepts $C$ introduced so far have been \emph{crisp} in that each point $z$ strictly either satisfies $(z \in C)$ or fails to satisfy $(z \notin C)$ the concept. However human concepts are typically understood to be instead \emph{fuzzy} or \emph{graded}, with membership taking some value in $[0,1]$. Fuzzy concepts are also most natural in machine learning, such as in the VAEs explored here, allowing more readily for  learning via gradient descent.


Formally, a fuzzy concept is given by a function 
\[
C \colon Z \to [0,1]
\]
For $z \in Z$, the value $C(z)$ represents the degree to which $z$ satisfies the concept, with $0$ meaning  not at all satisfied, and $1$ totally satisfied (a \emph{prototype} of the concept). If fuzzy concepts are to respect the structure of  conceptual space appropriately, they should not be arbitrary such mappings, but those which generalise convex subsets in some sense. One of the authors has recently proposed the following definition. 

%Todo: We may ultimately not want to mention log-concavity since it is no longer satisfied by e.g. mixtures of Gaussians (I expect). 
\begin{definition} \cite{tull2021categorical}
A \emph{fuzzy concept} of $Z$ is a measurable function $C \colon Z \to [0,1]$ which is \emph{log-concave}, meaning that 
\[
C(pz + (1-p)z') \geq C(z)^pC(z')^{1-p}
\]
\end{definition} 

In \cite{tull2021categorical} this definition is justified as the simplest which is compositionally well-behaved and includes crisp concepts (via their indicator functions $1_C$) and Gaussians as special cases. In this work we focus solely on the latter kind. 

Another common perspective on fuzzy concepts is to view them as probability distributions over $Z$. Formally, any fuzzy concept $C \colon Z \to [0,1]$ may, after suitable normalisation, be viewed as a density function for a probability measure
\begin{equation} \label{eq:fuzzy-density} 
p(z \mid C) := \frac{1}{\kappa} C(z) 
\end{equation} 
where $\kappa = \int_Z C(z) dz$ (provided this is non-zero and finite). The corresponding probability measure is then given by \[P(A\mid C) := \int_A p(z\mid C) dz\]
for each measurable subset $A \subseteq Z$. Intuitively, sampling from this distribution will produce points $z \in Z$ which are likely to fit the concept well, in that $p(z \mid C)$ (or equivalently $C(z)$) is high. 

In this work we consider only fuzzy concepts of the following form.

%  %Todo: We could mention that crisp concepts count as fuzzy ones, via their indicator functions, but this is not necessary for this article really. 
% \begin{example} 
% Any crisp concept $M \subseteq Z$ defines a fuzzy concept via its indicator function $C=1_M$, with $C(z) = 1$ iff $z \in M$, and $C(z) = 0$ otherwise.
% \end{example} 

% In this work we will restrict attention to fuzzy concepts of the following familiar kind. 

%Todo: this is just a single variable Gaussian!
\begin{example} 
We may define a fuzzy concept $C \colon Z \to [0,1]$ on $Z=\mathbb{R}^n$ from any multivariate Gaussian 
\begin{align} \label{eq:Gaussian} 
C(z;\mu,\Sigma) &= e^{-\frac{1}{2}(z - \mu)^{\mathsf{T}}\Sigma^{-1}(z -\mu)} \\ 
& = e^{\sum^n_{i=1}-\frac{1}{2 \sigma_i^2}(z_i - \mu_i)^2}
\end{align}  
with mean $\mu$ and covariance matrix $\Sigma$. In the second line we restrict to the case where $\Sigma$ is diagonal, with $i$-th diagonal entry $\sigma_i^2$. Probabilistically this corresponds to a multivariate normal distribution $p(z \mid C)$ as in \eqref{eq:fuzzy-density} with $\kappa =\sqrt{\prod^n_{i=1} 2 \pi \sigma_i^2}$.

 Note that in this case where $\Sigma$ is diagonal, any such Gaussian concept $C$ simply corresponds to a product of one-dimensional Gaussians, one per dimension. 
 \[
 C(z; \mu, \Sigma) = \prod^n_{i=1} C(z_i;\mu_i,\sigma_i^2)
 \]
 These for example include the concepts for composite concepts in the conceptual VAE. For a concept such as $C=$(Large, Yellow, Circle, Top), interpreted as `Large yellow circle at the top' we have  \Seanmar{Choose one of these equations}
\[
p(z \mid C)
=
p(z_1 \mid \text{Large }) p(z_2 \mid \text{Yellow }) p(z_3 \mid \text{Circle }) p(z_4 \mid \text{Top })
\]

 \[
C(z)
=
C(z_1;\mu_{\text{Large}},\sigma_{\text{Large}}^2) 
C(z_2;\mu_{\text{Yellow}},\sigma_{\text{Yellow}}^2) 
C(z_3;\mu_{\text{Circle}},\sigma_{\text{Circle}}^2) 
C(z_4;\mu_{\text{Top}},\sigma_{\text{Top}}^2) 
\]
 \end{example} 


\subsection{Composing concepts}

\Stevemar{I would have anything about composition earlier in the section, or perhaps future work, since finishing with the gaussian formulation above is a really nice way to finish off the section}

% Our choice of representation of fuzzy concepts is motivated by the  \emph{category-theoretic} treatment of conceptual spaces presented in \cite{bolt2019interacting} and extended to fuzzy concepts in \cite{tull2021categorical}. 


In \cite{tull2021categorical} our definition of fuzzy concepts is also extended to more general fuzzy \emph{conceptual processes} which transform concepts on conceptual one space to another, and formally define a \emph{symmetric monoidal category}. This builds on the earlier categorical treatment of crisp concepts in \cite{bolt2019interacting}. 

The categorical approach allows us to reason about and \emph{compose} concepts using simple \emph{string diagrams}. For example, the concepts in this work are given by composing  concepts from each domain, as below.
\[
\includegraphics[scale=0.25]{figs/9.png}
\]
% \[
% \begin{tikzpicture}
% 	\begin{pgfonlayer}{nodelayer}
% 		\node [style=map] (0) at (-6.75, 0.5) {large yellow square at top};
% 		\node [style=none] (1) at (-6.75, -1) {};
% 		\node [style=label] (2) at (-6.75, -1.5) {$Z$};
% 		\node [style=none] (3) at (-1.5, 0) {$=$};
% 		\node [style=map] (4) at (1, 0.5) {large};
% 		\node [style=none] (5) at (1, -1) {};
% 		\node [style=label] (6) at (1, -1.5) {Size};
% 		\node [style=map] (7) at (3.5, 0.5) {yellow};
% 		\node [style=none] (8) at (3.5, -1) {};
% 		\node [style=label] (9) at (3.5, -1.5) {Col};
% 		\node [style=map] (10) at (6, 0.5) {square};
% 		\node [style=none] (11) at (6, -1) {};
% 		\node [style=label] (12) at (6, -1.5) {Shape};
% 		\node [style=map] (13) at (8.5, 0.5) {top};
% 		\node [style=none] (14) at (8.5, -1) {};
% 		\node [style=label] (15) at (8.5, -1.5) {Pos};
% 	\end{pgfonlayer}
% 	\begin{pgfonlayer}{edgelayer}
% 		\draw (1.center) to (0);
% 		\draw (4) to (5.center);
% 		\draw (7) to (8.center);
% 		\draw (10) to (11.center);
% 		\draw (13) to (14.center);
% 	\end{pgfonlayer}
% \end{tikzpicture}
% \]
% Mathematically, this is because we use Gaussians with diagonal covariance matrices, which are (up to normalisation) products of Gaussians on each domain.
However, more general concepts on the overall space needn't factor as above. For example, we might imagine the concept of a `star' which depends on both size and colour, and which is such that a red star tends to be large and blue one to be small.
% \[
% \begin{tikzpicture}
% 	\begin{pgfonlayer}{nodelayer}
% 		\node [style=none] (0) at (0.5, 0.5) {};
% 		\node [style=medium map] (1) at (1.5, 1) {star};
% 		\node [style=none] (2) at (2.5, 0.5) {};
% 		\node [style=none] (3) at (0.5, -1) {};
% 		\node [style=none] (4) at (2.5, -1) {};
% 		\node [style=label] (5) at (0.5, -1.5) {Size};
% 		\node [style=label] (6) at (2.5, -1.5) {Col};
% 	\end{pgfonlayer}
% 	\begin{pgfonlayer}{edgelayer}
% 		\draw (0.center) to (3.center);
% 		\draw (2.center) to (4.center);
% 	\end{pgfonlayer}
% \end{tikzpicture}
% \]
% % The concept is such that
% \[
% \begin{tikzpicture}
% 	\begin{pgfonlayer}{nodelayer}
% 		\node [style=none] (0) at (0.5, 0.5) {};
% 		\node [style=medium map] (1) at (1.5, 1) {star};
% 		\node [style=none] (2) at (2.5, 0.5) {};
% 		\node [style=map] (3) at (0.5, -1) {large};
% 		\node [style=none] (4) at (2.5, -1) {};
% 		\node [style=label] (5) at (-0.75, -0.25) {Size};
% 		\node [style=label] (6) at (2.5, -1.5) {Col};
% 		\node [style=none] (7) at (4.25, 0) {$=$};
% 		\node [style=map] (9) at (6.5, 1) {red};
% 		\node [style=none] (10) at (6.5, 0.5) {};
% 		\node [style=none] (12) at (6.5, -1) {};
% 		\node [style=label] (14) at (6.5, -1.5) {Col};
% 	\end{pgfonlayer}
% 	\begin{pgfonlayer}{edgelayer}
% 		\draw (0.center) to (3);
% 		\draw (2.center) to (4.center);
% 		\draw (10.center) to (12.center);
% 	\end{pgfonlayer}
% \end{tikzpicture}
% \qquad
% \begin{tikzpicture}
% 	\begin{pgfonlayer}{nodelayer}
% 		\node [style=none] (0) at (0.5, 0.5) {};
% 		\node [style=medium map] (1) at (1.5, 1) {star};
% 		\node [style=none] (2) at (2.5, 0.5) {};
% 		\node [style=map] (3) at (0.5, -1) {small};
% 		\node [style=none] (4) at (2.5, -1) {};
% 		\node [style=label] (5) at (-0.75, -0.25) {Size};
% 		\node [style=label] (6) at (2.5, -1.5) {Col};
% 		\node [style=none] (7) at (4.25, 0) {$=$};
% 		\node [style=map] (9) at (6.5, 1) {blue};
% 		\node [style=none] (10) at (6.5, 0.5) {};
% 		\node [style=none] (12) at (6.5, -1) {};
% 		\node [style=label] (14) at (6.5, -1.5) {Col};
% 	\end{pgfonlayer}
% 	\begin{pgfonlayer}{edgelayer}
% 		\draw (0.center) to (3);
% 		\draw (2.center) to (4.center);
% 		\draw (10.center) to (12.center);
% 	\end{pgfonlayer}
% \end{tikzpicture}
% \]
\[
\includegraphics[scale=0.25]{figs/8.png}
\]
% \[
% \begin{tikzpicture}
% 	\begin{pgfonlayer}{nodelayer}
% 		\node [style=none] (0) at (0.5, 0.5) {};
% 		\node [style=medium map] (1) at (1.5, 1) {star};
% 		\node [style=none] (2) at (2.5, 0.5) {};
% 		\node [style=none] (3) at (0.5, -1) {};
% 		\node [style=none] (4) at (2.5, -1) {};
% 		\node [style=label] (5) at (0.5, -1.5) {Size};
% 		\node [style=label] (6) at (2.5, -1.5) {Col};
% 	\end{pgfonlayer}
% 	\begin{pgfonlayer}{edgelayer}
% 		\draw (0.center) to (3.center);
% 		\draw (2.center) to (4.center);
% 	\end{pgfonlayer}
% \end{tikzpicture}
% \qquad 
% \text{s.t.}
% \qquad 
% \begin{tikzpicture}
% 	\begin{pgfonlayer}{nodelayer}
% 		\node [style=none] (3) at (4, 0.5) {};
% 		\node [style=medium map] (4) at (5, 1) {star};
% 		\node [style=none] (5) at (6, 0.5) {};
% 		\node [style=map] (6) at (4, -1) {small};
% 		\node [style=none] (7) at (6, -1) {};
% 		\node [style=none] (10) at (7.25, 0) {$=$};
% 		\node [style=map] (11) at (8.75, 1) {blue};
% 		\node [style=none] (12) at (8.75, 0.5) {};
% 		\node [style=none] (13) at (8.75, -1) {};
% 		\node [style=none] (14) at (11.75, 0.5) {};
% 		\node [style=medium map] (15) at (12.75, 1) {star};
% 		\node [style=none] (16) at (13.75, 0.5) {};
% 		\node [style=map] (17) at (11.75, -1) {large};
% 		\node [style=none] (18) at (13.75, -1) {};
% 		\node [style=none] (19) at (15, 0) {$=$};
% 		\node [style=map] (20) at (16.5, 1) {red};
% 		\node [style=none] (21) at (16.5, 0.5) {};
% 		\node [style=none] (22) at (16.5, -1) {};
% 	\end{pgfonlayer}
% 	\begin{pgfonlayer}{edgelayer}
% 		\draw (3.center) to (6);
% 		\draw (5.center) to (7.center);
% 		\draw (12.center) to (13.center);
% 		\draw (14.center) to (17);
% 		\draw (16.center) to (18.center);
% 		\draw (21.center) to (22.center);
% 	\end{pgfonlayer}
% \end{tikzpicture}
% \]
The diagrammatic approach is useful for combining these more general concepts. A common approach is to use their pointwise product, which appears in diagrams through white `copying' dots. In \cite{bolt2019interacting} these combinations are applied to crisp concepts to give conceptual semantics for natural language, by converting sentences into concepts diagrammatically as below.  Note that these diagrammatic concept combinations do not require any learning beyond the concepts themselves.
\[
\includegraphics[scale=0.18]{figs/3.png}
= 
\includegraphics[scale=0.18]{figs/4.png}
\]
% \end{equation} 
% Another form of concept combination, which can be seen to generalise the above, is given by pointwise multiplication of concepts on the same space. 
% \[
% \begin{tikzpicture}
% 	\begin{pgfonlayer}{nodelayer}
% 		\node [style=whitedot] (0) at (0, -0.5) {};
% 		\node [style=map] (1) at (-1, 0.75) {$C_1$};
% 		\node [style=map] (2) at (1, 0.75) {$C_2$};
% 		\node [style=none] (3) at (0, -1.5) {};
% 	\end{pgfonlayer}
% 	\begin{pgfonlayer}{edgelayer}
% 		\draw [bend right=45] (1) to (0);
% 		\draw [bend left=45] (2) to (0);
% 		\draw (3.center) to (0);
% 	\end{pgfonlayer}
% \end{tikzpicture}
% \]
% In \cite{bolt2019interacting} this categorical approach to combining (crisp) concepts is used to give conceptual semantics for natural language, by converting sentences into concepts diagrammatically as below. 
% \begin{equation} \label{eq:fruit-bitter}
% \includegraphics[scale=0.2]{figs/3.png}
% = 
% \includegraphics[scale=0.2]{figs/4.png}
% \end{equation} 
 In future work it would be interesting to explore the learning of non-factored concepts in our setup, as well as the effectiveness of these formal composition procedures. Beyond this, the categorical approach allows one to explore the learning of conceptual processes between domains, such the `metaphorical' mappings suggested in \cite{tull2021categorical} between taste and colour spaces. 
 \[
\includegraphics[scale=0.2]{figs/6.png}
\qquad 
\includegraphics[scale=0.2]{figs/7.png}
\]
\Seanmar{Maybe leave out metaphor part}

